Sampling with collective variables: Relative error analysis for umbrella sampling under general conditions

We consider the problem of estimating the expectation of a function (observable) with respect to a high-dimensional probability distribution, under the assumption that a low-dimensional collective variable map captures all the directions of slow mixing for the distribution. More precisely, under the assumption that the fibers of the collective variable map satisfy a log-Sobolev inequality, we establish non-asymptotic relative-error guarantees for this problem using the eigenvector method for umbrella sampling (EMUS). Our analysis applies to both log-Lipschitz observables and indicator of convex sets, and gives complexity bounds that are polynomial in regularity parameters and inverse relative accuracy, and exponential in the dimension of the collective variable space. As a relative error guarantee, our bounds apply to rare event estimation. We consider Gaussian biasing windows defined on a low-dimensional collective variable space and analyze a modified sparse matrix version of EMUS. The bounds quantify the effect of the map through mixing of the conditional distribution and fluctuation of the observable along the fibers.

==> Gaussian_Sampling.tex <==
In this subsection, we derive a sufficient run time to obtain samples from $\nu_k \propto \pi_k|_{K_u}$ such that such that Assumption \ref{a: main} (2) is satisfied with $\chi^2(\tilde{\nu}_k,\nu_k) \leq \tilde{\epsilon}$. 
Under Assumptions \ref{a: Gaussian Windows} the windows $\psi_k$ are Gaussian and the log potential $\pi(x)$ is $\ell$-smooth, therefore the tilted measure $\pi_k$ satisfies a log Sobolev inequality. Crucially, the restricted measure $\nu_k$ inherits this property with the same constant, ensuring that the restriction to the influence set does not degrade the resulting mixing time.

We note that under these assumptions, it's possible to sample from any window naively by initializing samples from $\psi_i(x)$ and running a Markov chain with stationary distribution $\nu_i(x) \propto \psi_i(x)\pi(x) 1_{K_U}$.
However, the convergence bounds for this method depend on the gradient of the potential at the gaussian centers, i.e. $\left\|\nabla V(y_k) \right\|$. 
To control this error, the inverse temperature $\beta$ must be large (requiring extremely narrow windows). Additionally, because the chain targets the restricted distribution $\nu_i$, naive initialization requires discarding any initial samples from $\psi_i(x)$ that fall outside $K_u$. 
For padding windows whose center lie far outside $K_u$, this rejection based initialization becomes computationally bad.


Instead, by leveraging Assumption \ref{a: main} (1), we propose sampling from the windows inductively.
Under the good path assumption initial samples from window $i$ can be used as a warm start to sample from a neighboring window $i+1$.
To avoid the computational cost of rejection-based initialization in the padding region, we initialize the process in window $k^*$ which is interior to $K_u$. 
The main result Proposition \ref{p: gaussian mixing time} provides a convergence guarantee for drawing samples from any specific window, given its respective initialization. 

\begin{proposition}\label{p: gaussian mixing time}
     Let Assumptions \ref{a: main}, \ref{a: Gaussian Windows} and \ref{a: Gaussian windows 2} hold. 
     Let $\nu_i = \pi_i|_{K_u}$ be the measure restricted to $K_u \subseteq A$.
     Let $\tilde{\nu}_k$ be the distribution obtained after running a reversible Markov process $P_T^{(k)}$ with stationary distribution $\nu_k$ for time $T$ on the restricted set $K_u$. 
     Suppose the windows are arranged such that there exists a path of length at most $L$, $(k_0, \dots, k_L)$, such that the starting window $k_0$ satisfies $\|\nabla V(y_{k_0})\| \le G$ (Base Case) and every adjacent pair $(k_{i-1}, k_i)$ satisfies the overlap condition (Assumption \ref{a: main}(1)). 
     Define the initialization bias $\mathcal{E}_0 \vcentcolon = \left(\frac{\beta}{\beta-\ell} \right)^d\exp(\frac{G^2}{\beta-\ell}) -1$ and the window overlap factor $\mathcal{A} \vcentcolon = \exp(\frac{\beta^2\Delta^2}{2(\beta - \ell)})$, where $\Delta = \|y_{k+1} - y_k\|$ for windows $k+1$, $k$ along the good path. Then for any $\tilde{\epsilon} > 0$ choosing 
     $$T_{mix} \geq \frac{1}{2(\beta - \ell)}\max\left\{\frac{1}{2}\log(3), \log\left(\frac{\mathcal{A}(\tilde{\epsilon} +1)-1}{\tilde{\epsilon}}\right),\log\left(\frac{\mathcal{E}_0}{\tilde{\epsilon}}\right) \right\}$$
     yields $\chi^2(\tilde{\nu}_k, \nu_k) \leq \tilde{\epsilon}$, for all $k \in [1,L]$.
\end{proposition}
% \begin{lem}\label{l: LSI bound gaussian}(LSI Constant Bound) Let Assumption \ref{a: Gaussian windows 2}  hold, so that $\pi(x) \propto e^{-V(x)}$ has an $\ell$-smooth potential and $\psi_k(x) \propto \exp(-{\frac{\beta}{2}}\left\|x-y_k\right\|^2).$ If the Gaussian temperature is chosen such that $\beta > \ell$ then $\pi_k \propto \psi_k\pi$ satisfies a log Sobolev constant $C_{LS}$ given by: 

% $$C_{LS} \leq \frac{1}{\beta-\ell}.$$
% \end{lem}
\begin{proof}
    $\pi_k \propto \psi_k \pi$ implies $-\log \pi_k = \frac{\beta}{2}\left\|x-y_k\right\|^2 + V(x) + \log Z_k$. Therefore, by $\ell$-smoothness, 
    $$\nabla^2V_k(x) =  \beta I +\nabla^2V(x) \succeq \left(\beta - \ell\right)I.$$
    Strong log-concavity implies the LSI bound by the Bakry-\'Emery criterion. 
\end{proof}
    
\begin{lem}(Warm Start Propogation \& Initialization)\label{l: warm_start_propogation_gaussian} Let Assumptions \ref{a: Gaussian Windows} and \ref{a: Gaussian windows 2} hold. Let the windows $\psi_k(x)$ be Gaussians with temperature $\beta > \ell$ and centers $\{y_k\}$. Lastly, let $\nu_i = \pi_i|_{K_u}$ be the measure restricted to $K_u \subseteq A$. 
\begin{enumerate}
    \item (Inductive Initialization) Suppose window $i$ has $i'$ such that $h = y_i - y_{i'}$ and $\|h\| = \Delta$. If we initialize the MCMC chain for $\nu_i$ using samples from $\nu_{i'}$, then the $\chi^2$-divergence satisfies: 
    $$\chi^2(\nu_{i'}, \nu_i) \leq \exp(\frac{\beta^2\Delta^2}{\beta-\ell})-1.$$
    \item (Base Initialization) Suppose there exists a Gaussian window $\psi_{k^*}$ with center $y_{k^*}$ such that $\|\nabla V(y_{k^*})\| \leq \delta$. If we initialize the MCMC chain for $\pi_{k^*}|_{K_u}$ using samples from $\mu_0 \propto \psi_{k^*}|_{K_u}$, then the $\chi^2$-divergence satisfies: 
    $$\chi^2(\mu_0, \pi_{k^*}) \leq \left(\frac{\beta}{\beta-\ell}\right)^d\exp(\frac{\delta^2}{\beta - \ell})-1.$$
\end{enumerate}
\end{lem}
\begin{proof} We will prove each part separately: 

    \begin{enumerate}
        \item \textit{(Proof of Inductive Initialization)} Let $\nu_i(x) = \frac{1}{Z_i}e^{-V(x)}\psi_i(x)$ and $\nu_{i'}(x) = \frac{1}{Z_{i'}}e^{-V(x)}\psi_{i'}(x)$. The $\chi^2$ divergence is then given by 
        $$\chi^2(\nu_{i'}, \nu_i) +1 = \frac{Z_i}{Z_{i'}}\mathbb{E}_{\nu_{i'}}\left[\frac{\psi_i(x)}{\psi_{i'}(x)} \right].$$
        Furthermore, we can express the ratio of the partition functions as 
        $$\frac{Z_i}{Z_{i'}} = \frac{1}{Z_{i'}}\int_{K_u} e^{-V(x)}\psi_i(x)dx = \int_{K_u} \frac{\psi_i(x)}{\psi_{i'}(x)}e^{-V(x)}\frac{\psi_{i'}(x)}{Z_{i'}}dx = \mathbb{E}_{\nu_{i'}}\left[\frac{\psi_i(x)}{\psi_{i'}(x)}\right].$$
        Defining $r(x) =\frac{\psi_i(x)}{\psi_{i'}(x)}$ we have that
         $$\chi^2(\nu_{i'}, \nu_i) +1 = \mathbb{E}_{\nu_{i'}}\left[r(x)\right]\mathbb{E}_{\nu_{i'}}\left[\frac{1}{r(x)}\right].$$
Recalling that $h = y_i - y_{i'}$, the ratio r(x) simplifies to: 
$$r(x) = \exp(-\frac{\beta}{2}\left(\|x-y_i\|^2 - \|x-y_{i'}\|^2 \right))= \exp(\beta\langle x-y_{i'},h \rangle-\frac{\beta}{2}\|h\|^2).$$
We note that $\nu_{i'}$ satisfies and LSI with $C_{LS} \leq \frac{1}{\beta - \ell}$ (Lemma \ref{l: LSI bound gaussian}). Then, applying Lemma \ref{l: herbst argument} to the $\|h\|$-Lipschitz function $f(x) = \langle h,x\rangle$, 
\begin{align*}
\mathbb{E}_{\nu_{i'}}\left[r(x)\right]&= \exp(\beta\langle \mathbb{E}_{\nu_{i'}}[x]-y_{i'} ,h\rangle-\frac{\beta}{2}\|h\|^2)\mathbb{E}_{\nu_{i'}}\left[e^{\beta\langle h, x -\mathbb{E}_{\nu_{i'}}[x]\rangle}\right]\leq\exp(\beta\langle \mathbb{E}_{\nu_{i'}}[x]-y_{i'} ,h\rangle-\frac{\beta}{2}\|h\|^2+\frac{\beta^2\|h\|^2}{2(\beta-\ell)})\\
\mathbb{E}_{\nu_{i'}}\left[\frac{1}{r(x)}\right]&= \exp(-\beta\langle \mathbb{E}_{\nu_{i'}}[x]-y_{i'} ,h\rangle+\frac{\beta}{2}\|h\|^2)\mathbb{E}_{\nu_{i'}}\left[e^{\beta\langle h, x -\mathbb{E}_{\nu_{i'}}[x]\rangle}\right]\leq\exp(-\beta\langle \mathbb{E}_{\nu_{i'}}[x]-y_{i'} ,h\rangle+\frac{\beta}{2}\|h\|^2+\frac{\beta^2\|h\|^2}{2(\beta-\ell)}). 
\end{align*}
Then we have that 
$$\chi^2(\nu_{i'}, \nu_i) +1 = \mathbb{E}_{\nu_{i'}}\left[r(x)\right]\mathbb{E}_{\nu_{i'}}\left[\frac{1}{r(x)}\right] \leq \exp(\frac{\beta^2\|h\|^2}{\beta-\ell}).$$
\item \textit{(Proof of Base Initialization)} Let $\nu_{k^*}(x) = \frac{1}{Z_{k^*}}e^{-V(x)}\psi_{k^*}(x)$ and $\mu_0 = \mathcal{N}(y_{k^*}, \beta^{-1}I)|_{K_u}$ and $Z_{\mu_{\beta}} = \int_{K_u} \mu_0(dx)$. The $\chi^2$ divergence is then given by 
$$\chi^2(\mu_0, \pi_{k^*}) +1 = \frac{Z_{k^*}}{Z_{\mu_\beta}}\mathbb{E}_{\mu_0}\left[e^{V(x)}\right].$$
Moreover, since $\mu_0 \propto \psi_{k^*}$, we can express the ratio of partition functions as 
$$\frac{Z_{k^*}}{Z_{\mu_\beta}} = \frac{1}{Z_{\mu_\beta}}\int e^{-V(x)}\psi_{k^*}(x)dx=\mathbb{E}_{\mu_0}\left[e^{-V(x)} \right].$$
Therefore we can express the $\chi^2$ as 
$$\chi^2(\mu_0, \pi_{k^*}) +1 =\mathbb{E}_{\mu_0}\left[e^{-V(x)} \right]\mathbb{E}_{\mu_0}\left[e^{V(x)}\right].$$
By the $\ell$-smoothness of $V(x)$, we have that
$$   V(y_{k^*}) + \langle \nabla V(y_{k^*}), x-y_{k^*} \rangle - \frac{\ell}{2}\|x-y_{k^*}\|^2 \leq V(x) \leq V(y_{k^*}) + \langle \nabla V(y_{k^*}), x-y_{k^*} \rangle + \frac{\ell}{2}\|x-y_{k^*}\|^2.$$
Using $\ell$-smoothness and letting $\mu^* = \mathcal{N}(y_{k^*},(\beta-\ell)^{-1}I_d)$ we get the following upper bounds: 
\begin{align*}
    \mathbb{E}_{\mu_0}\left[e^{-V(x)} \right]&\leq e
    ^{-V(y_{k^*})}\mathbb{E}_{\mu_0}\left[e
    ^{- \langle \nabla V(y_{k^*}), x-y_{k^*} \rangle + \frac{\ell}{2}\|x-y_{k^*}\|^2} \right]=e
    ^{-V(y_{k^*})}\frac{Z_{\mu_{\beta-\ell}}}{Z_{\mu_\beta}}\mathbb{E}_{\mu^*}\left[e^{- \langle \nabla V(y_{k^*}), x-y_{k^*}\rangle} \right] \\ 
    \mathbb{E}_{\mu_0}\left[e^{V(x)}\right]&\leq e
    ^{V(y_{k^*})}\mathbb{E}_{\mu_0}\left[e
    ^{\langle \nabla V(y_{k^*}), x-y_{k^*} \rangle + \frac{\ell}{2}\|x-y_{k^*}\|^2} \right]=e
    ^{V(y_{k^*})}\frac{Z_{\mu_{\beta-\ell}}}{Z_{\mu_\beta}}\mathbb{E}_{\mu^*}\left[e^{\langle \nabla V(y_{k^*}), x-y_{k^*}\rangle} \right].
\end{align*}
$\mu^*$ is Gaussian and therefore satisfies an LSI with $C_{LS} = \frac{1}{\beta-\ell}$. Then applying Lemma \ref{l: herbst argument} with $\|\nabla V(y_{k^*})\|$-Lipschitz function $f(x) = \langle\nabla V(y_{k^*}),x-y_{k^*}\rangle$, 
\begin{align*}
    \mathbb{E}_{\mu_0}\left[e^{-V(x)}\right] &\leq e
    ^{-V(y_{k^*})}\frac{Z_{\mu_{\beta-\ell}}}{Z_{\mu_\beta}}e^{\frac{\|\nabla V(y_{k^*})\|^2}{2(\beta-\ell)}}\\
     \mathbb{E}_{\mu_0}\left[e^{V(x)}\right] &\leq e
    ^{V(y_{k^*})}\frac{Z_{\mu_{\beta-\ell}}}{Z_{\mu_\beta}}e^{\frac{\|\nabla V(y_{k^*})\|^2}{2(\beta-\ell)}}.
\end{align*}
Lastly, applying  $\frac{Z_{\mu_{\beta-\ell}}}{Z_{\mu_\beta}} \leq \left( \frac{\beta}{\beta-\ell}\right)^\frac{d}{2}$ and $\| \nabla V(y_{k^*})\| \leq \delta$ to the product yields
$$\chi^2(\nu_0, \pi_{k^*}) +1 \leq \left(\frac{\beta}{\beta-\ell}\right)^d\exp(\frac{\|\nabla V(y_{k^*})\|^2}{\beta-\ell})\leq\left(\frac{\beta}{\beta-\ell}\right)^d\exp(\frac{\delta^2}{\beta-\ell}).$$
    \end{enumerate}
\end{proof}
\begin{lem}(Inductive Stability of Restricted Initialization Error) \label{l: inductive stability initialization gaussian} 
Let Assumption $\ref{a: Gaussian windows 2}$ hold with $\beta > \ell$.  Let $\nu_i = \pi_i|_{K_u}$ be the measure restricted to $K_u \subseteq A$.
Let $\tilde{\nu}_{k-1}$ be the distribution obtained after running a reversible restricted Markov process $P_{T}^{(k-1)}$ on $K_U$ with stationary distribution $\nu_{k-1}$ for time $T$. Assume that $P_{T}^{(k-1)}$ is initialized with samples from $\tilde{\nu}_{k-2}$ so that $\chi^2(\tilde{\nu}_{k-2}, \nu_{k-1}) \leq {\epsilon}$. If window $k$ is the neighbor of $k-1$ satisfying Lemma \ref{l: warm_start_propogation_gaussian} (1) then 
$$\chi^2(\tilde{\nu}_{k-1}, \nu_k)\leq (1 + \epsilon)\exp\left(\frac{\beta^2\left\|h\right\|^2}{2(\beta - \ell)}\right)-1$$
provided that $T \geq \frac{1}{4(\beta - \ell)}\log(3)$.
\end{lem}

\begin{proof} We note that the base case is satisfied by Lemma \ref{l: warm_start_propogation_gaussian} (2) so it's left to show the inductive case. 
    Expressing the $\chi^2$ divergence as  $\chi^2(\tilde{\nu}_{k-1},\nu_k) +1 = \mathbb{E}_{\nu_k}\left(\frac{d\tilde{\nu}_{k-1}}{d\nu_k} \right)^2$ and by the change of measure $d\nu_k = \frac{d\nu_k}{d\nu_{k-1}}d\nu_{k-1}$ yields 
    $$\chi^2(\tilde{\nu}_{k-1},\nu_k) +1 = \mathbb{E}_{\nu_{k-1}}\left[\left(\frac{d\tilde{\nu}_{k-1}}{d\nu_k} \right)^2\frac{d\nu_k}{d\nu_{k-1}}\right]=\mathbb{E}_{\nu_{k-1}}\left[\left(\frac{d\tilde{\nu}_{k-1}}{d\nu_{k-1}} \right)^2\frac{d\nu_{k-1}^2}{d\nu_k^2}\frac{d\nu_k}{d\nu_{k-1}}\right] = \mathbb{E}_{\nu_{k-1}}\left[\left(\frac{d\tilde{\nu}_{k-1}}{d\nu_{k-1}} \right)^2\frac{d\nu_{k-1}}{d\nu_{k}}\right].$$ Applying Holder's inequality yields
    $$\mathbb{E}_{\nu_{k-1}}\left[\left(\frac{d\tilde{\nu}_{k-1}}{d\nu_{k-1}} \right)^2\frac{d\nu_k}{d\nu_{k-1}}\right] \leq \left\|\frac{d\tilde{\nu}_{k-1}}{d\nu_{k-1}} \right\|_{L^4(\nu_{k-1})}^2\left\|\frac{d\nu_{k-1}}{d\nu_k}\right\|_{L^2(\nu_{k-1})}.$$
    The second term is bounded $\exp(\frac{\beta^2\Delta^2}{2(\beta - \ell)})$ per Lemma \ref{l: warm_start_propogation_gaussian} (1). 
    For the first term, since the process $P^{(k-1)}$ is reversible with respect to $\nu_{k-1}$, we can express $\frac{d\tilde{\nu}_{k-1}}{d\nu_{k-1}} = \frac{dP_{T}^{(k-1)}{\tilde{\nu}}_{k-2}}{d\nu_{k-1}}= P_{T}^{(k-1)}\frac{d\tilde{\nu}_{k-2}}{d\nu_{k-1}}.$ Therefore by Hypercontractivity (Lemma \ref{l: gross_hypercontractive}), with $T > \frac{C_{LS}}{4}\log(3)$, 
    $$\left\|\frac{d\tilde{\nu}_{k-1}}{d\nu_{k-1}} \right\|_{L^4(\nu_{k-1})}^2= \left\| P_{T}^{(k-1)}\frac{d\tilde{\nu}_{k-2}}{d\nu_{k-1}} \right\|_{L^4(\nu_{k-1})}^2 \leq \left\| \frac{d\tilde{\nu}_{k-2}}{d\nu_{k-1}} \right\|_{L^2(\nu_{k-1})}^2 = \chi^2(\tilde{\nu}_{k-2}, \nu_{k-1}) +1 < \epsilon + 1.$$
    Combining the bounds and noting that, by Lemma \ref{l: LSI bound gaussian}, $C_{LS} \leq \frac{1}{\beta - \ell}$, yields the result. 
\end{proof}
\begin{proof}[\textit{Proof of Proposition \ref{p: gaussian mixing time}}] Since for any path there exists $k^*$ satisfying  $\|\nabla V(y_{k_0}) \| \leq \delta$ this satisfies the base case initialization assumptions, combined with Lemma \ref{l: warm_start_propogation_gaussian} and \ref{l: chisq MCMC} yields
$$\chi^2(\tilde{\nu}_{k_1}, \nu_{k_1}) \leq e^\frac{-2T}{C_{LS}}\chi^2(\mu_0,\nu_{k_1}) \leq e^\frac{-2T}{C_{LS}}\mathcal{E}_0.$$
Where we use $C_{LS} \leq \frac{1}{\beta - \ell}$ as in Lemma \ref{l: LSI bound gaussian}. Setting this less than $\tilde{\epsilon}$ and solving for $T$ yields $T \geq \frac{1}{2(\beta-\ell)}\log\left(\frac{\mathcal{E}_0}{\tilde{\epsilon}}\right).$ 

In the case of the inductive error stability the results follow directly from Lemma \ref{l: inductive stability initialization gaussian} and \ref{l: chisq MCMC} which yield 
$$\chi^2(\tilde{\nu}_{k_i}, \nu_{k_i}) \leq e^\frac{-2T}{C_{LS}}\chi^2(\mu_0,\nu_{k_i}) \leq e^\frac{-2T}{C_{LS}}(1+\tilde{\epsilon})\mathcal{A} - 1.$$
Setting this to be less than $\tilde{\epsilon}$ and solving for $T$ yields $T \geq \frac{1}{2(\beta-\ell)}\log\left(\frac{\mathcal{A}(1+\tilde{\epsilon})-1}{\tilde{\epsilon}}\right)$. Lastly, noting that Lemma \ref{l: inductive stability initialization gaussian} requires $T \geq \frac{1}{4(\beta - \ell)}\log(3)$ yields the final result. 

\end{proof}

==> Proof_sketch.tex <==
This is just a first pass at a proof sketch. Using all the notation from Section 1 and defining
\begin{align*}
    \bar{A} &= \sum_{k=1}^L \bar{w}_k \bar{g}^*_k, &&\bar{B}=  \sum_{k=1}^L \bar{w}_k \bar{1}^*_k\\
    \tilde{A}_{\bar{w}} &= \sum_{k=1}^L \bar{w}_k \mathbb{E}_{\tilde{\pi}_k}[g^*],   &&\tilde{B}_{\bar{w}}= \sum_{k=1}^L\bar{w}_k\mathbb{E}_{\tilde{\pi}_k}[1^*]\\
    \tilde{A}_{w} &= \sum_{k=1}^L w_k \mathbb{E}_{\tilde{\pi}_k}[g^*],   &&\tilde{B}_{w}= \sum_{k=1}^Lw_k\mathbb{E}_{\tilde{\pi}_k}[1^*]\\
     A &= \sum_{k=1} w_k \mathbb{E}_{\pi_k}[g^*],   &&B= \sum_{k=1} w_k \mathbb{E}_{\pi_k}[1^*]
\end{align*}
Where $w_k$ are the true weights and our $N_k$ samples $\{x_i^k\} \sim \tilde{\pi}_k$. Then using this notation, 
\begin{align*}
    |\log \bar{\pi}(g) - \log \pi(g)| &= |\log\frac{\bar{A}}{\bar{B}} - \log\frac{A}{B}|\\
    &= |\log\frac{\bar{A}}{\bar{B}} - \log\frac{\tilde{A}_{\bar{w}}}{\tilde{B}_{\bar{w}}} +\log\frac{\tilde{A}_{\bar{w}}}{\tilde{B}_{\bar{w}}} -\log\frac{\tilde{A}_{w}}{\tilde{B}_{w}} + \log\frac{\tilde{A}_{w}}{\tilde{B}_{w}} - \log\frac{A}{B}|\\
    &\leq |\log\frac{\bar{A}}{\bar{B}} - \log\frac{\tilde{A}_{\bar{w}}}{\tilde{B}_{\bar{w}}}| +  |\log\frac{\tilde{A}_{\bar{w}}}{\tilde{B}_{\bar{w}}} -\log\frac{\tilde{A}_{w}}{\tilde{B}_{w}}|+|\log\frac{\tilde{A}}{\tilde{B}} - \log\frac{A}{B}|.
\end{align*}
\begin{enumerate}
    \item {\bf Controlling numerical approximation error $|\log\frac{\bar{A}}{\bar{B}} - \log\frac{\tilde{A}}{\tilde{B}}| \leq 2\log C_1$:} 
    
    This reduces to $|\frac{\bar{f}^*_k}{\mathbb{E}_{\tilde{\pi}_k} [f^*]}| \leq C_1$.
    Applying definitions and the triangle inequality yields, 
    \begin{align*}
|\log\frac{\bar{A}}{\bar{B}} - \log\frac{\tilde{A}}{\tilde{B}}|& \leq |\log\frac{\sum_k \bar{w}_k\bar{g}^*_k}{\sum_k \bar{w}_k \mathbb{E}_{\tilde{\pi}_k}[g^*]}| + |\log\frac{\sum_k \bar{w}_k\bar{1}^*_k}{\sum_k \bar{w}_k \mathbb{E}_{\tilde{\pi}_k}[1^*]}|. 
    \end{align*}
For a general $f$ that includes $g$ and $1$ we then require an upper bound on $|\log\frac{\sum_k \bar{w}_k\bar{f}^*_k}{\sum_k \bar{w}_k\mathbb{E}_{\tilde{\pi}_k}[f^*]}|$. 

Then since $$\frac{\sum_k A_k}{\sum_k B_k} = \frac{\sum_k B_k\frac{A_k}{B_k}}{\sum_k B_k} \leq C$$ for $ \max_k\frac{A_k}{B_k} \leq C$. We have
$$|\log\frac{\sum_k \bar{w}_k\bar{f}^*_k}{\sum_k \bar{w}_k\mathbb{E}_{\tilde{\pi}_k}[f^*]}| \leq \log C_1$$ 

for $|\frac{\bar{w}_k\bar{f}^*_k}{\mathbb{E}_{\bar{w}_k\tilde{\pi}_k} [f^*]}|= |\frac{\bar{f}^*_k}{\mathbb{E}_{\tilde{\pi}_k} [f^*]}| \leq C_1$. 
This term is bounded by standard Monte Carlo estimation error, $(1+ \epsilon)$ using Chernoff/Chebyshev. Notes: $1*$ is bounded however $g^*$ might not necessarily be bounded. 

\item {\bf Controlling weight error $|\log\frac{\tilde{A}_{\bar{w}}}{\tilde{B}_{\bar{w}}} -\log\frac{\tilde{A}_{w}}{\tilde{B}_{w}}|\leq 2\log C_2$:}
This reduces to  $|\frac{\bar{w}_k}{w_k}| \leq C_2$.
Proceeding in a similar fashion to (1) yields 
$$|\log\frac{\sum_k \bar{w}_k\mathbb{E}_{\tilde{\pi}_k}[f^*]}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}[f^*]}|\leq \log C_2$$
for $|\frac{\bar{w}_k\mathbb{E}_{\tilde{\pi}_k}[f^*]}{w_k\mathbb{E}_{\tilde{\pi}_k}[f^*] }| = |\frac{\bar{w}_k}{w_k}| \leq C_2.$


The $|\frac{\bar{w}_k}{w_k}|$ term, \note{assuming we can fit the setting of Thm. 3 in perturbation bounds paper,} can be bounded by 
$$|\frac{\bar{w}_k}{w_k}| = |\exp(\log \bar{w}_k - \log w_k)| \leq |\exp(C)|.$$

\textbf{Implementation of Theorem 3: }  Applying Theorem 3 from perturbations paper to bound relative weights with no exponential blow up. Theorem 3/Corollary 2 as written with the assumption that for all $i,j$ there exists a path $i= i_0, \dots, i_N = j$ s.t. $F_{i_ti_{t+1}}\geq c_p$ is not sufficient for good bounds. 

    Example: Define F to be the following chain with $c_p = \frac{1}{3}$

    \begin{figure}[h!]
\centering
\begin{tikzpicture}[
    node distance=1cm and 0.8cm,
    state/.style={circle, draw, thick, minimum size=7mm},
    every edge/.style={draw, -{Stealth[length=2mm]}},
    prob/.style={font=\footnotesize, sloped},
]
    % Define the chain of nodes
    \begin{scope}[start chain=auto]
        \foreach \i in {1,...,11} {
            \node[state, on chain] (s\i) {\i};
        }
    \end{scope}

    % --- Basin 1 (States 1-5) ---
    % Self-loop at 1
    \path (s1) edge [loop above, prob, "$2/3$"] (s1);
    % Edges for 1-4
    \foreach \i [evaluate=\i as \j using int(\i+1)] in {1,...,4} {
        \path (s\i) edge [bend left, prob, above, "$1/3$"] (s\j);
        \path (s\j) edge [bend left, prob, below, "$2/3$"] (s\i);
    }
    
    % --- Barrier (State 6) ---
    % 5 <-> 6
    \path (s5) edge [bend left, prob, above, "$1/3$"] (s6);
    \path (s6) edge [bend left, prob, below, "$1/2$"] (s5);
    % 6 <-> 7
    \path (s6) edge [bend left, prob, above, "$1/2$"] (s7);
    \path (s7) edge [bend left, prob, below, "$1/3$"] (s6);

    % --- Basin 2 (States 7-11) ---
    % Edges for 7-10
    \foreach \i [evaluate=\i as \j using int(\i+1)] in {7,...,10} {
        \path (s\i) edge [bend left, prob, above, "$2/3$"] (s\j);
        \path (s\j) edge [bend left, prob, below, "$1/3$"] (s\i);
    }
    % Self-loop at 11
    \path (s11) edge [loop above, prob, "$2/3$"] (s11);
    
\end{tikzpicture}
\caption{This chain has stationary distribution $\pi \propto [1, \frac{1}{2}, \frac{1}{4}, \frac{1}{8}, \frac{1}{16}, \frac{1}{24}, \frac{1}{16}, \frac{1}{8}, \frac{1}{4}, \frac{1}{2}, 1]$}
\end{figure}
with $\epsilon=.01$ the bound from Corollary 2 is computed as $\sum_{i \neq j} \frac{\epsilon}{Q_{ij}(S)} \approx 51.090587.$ Which gives us an exponentially bad bound on the relative weights. Also note that $\frac{Z_{i+1}}{Z_i} \in [\frac{1}{2},2].$

To address this we either need stronger assumptions on F or to better the bound from Theorem 3. 

\textbf{Solution: }I believe there is some hope in the following. Using $\chi^2$ and Chebyshev, this can be roughly expressed as, with probability $1-\delta$
\begin{align}\label{eq:F_ij error}
    |\bar{F}_{ij} - F_{ij}|&\leq |\bar{F}_{ij}-\tilde{F}_{ij}| + |\tilde{F}_{ij} - F_{ij}|\\
     &\leq \sqrt{Var_{\pi_i}(\psi_j^*(x))}\cdot\bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}} + \chi^2(\tilde{\pi}_i,\pi_i)^\frac{1}{2} \bigg)
\end{align}
This is to say that in the error bound from corollary 2, for i,j with little overlap,  $|\tilde{F}_{ij}-F_{ij}|$ is exponentially small when $Q_{ij}(S)$ is exponentially small. Therefore using $\epsilon$ as the worst case for every $F_{ij}$ is undesirable—instead we should be using some epsilon relative to the overlap.

Proceed as follows: 
\begin{enumerate}
    \item By Corollary 2,
        \begin{equation}
            ||\log w-\log\bar{w}||_\infty \leq \sum_{i\neq j}\frac{|\bar{F}_{ij} - F_{ij}|}{Q_{ij}(S)}.
        \end{equation}
    We apply the bound $Q_{ij}(S) \geq (1-\frac{1}{L})^{|i-j|}c_p^{|i-j|}$ ($\dagger$), 
    \begin{equation*}
            ||\log w-\log\bar{w}||_\infty \leq \sum_{i\neq j}\frac{|\bar{F}_{ij} - F_{ij}|}{ (1-\frac{1}{L})^{|i-j|}c_p^{|i-j|}}.
        \end{equation*}
        ($\dagger$) is satisfied by applying the definition $S_{ij} = \min(\bar{F}_{ij}, F_{ij})$ and then showing that by choice of $N$ and $T$ (if $\tilde{\pi}$ comes from a Markov process), $|\frac{\bar{F}_{ij}}{F_{ij}} - 1| \leq \frac{1}{L}$ with high probability. Which yields  that $\bar{F}_{ij} \geq (1 - \frac{1}{L})F_{ij}$. Since $F_{ij} \geq c_p$ along the good path we get the lower bound $S_{ij} \geq (1-\frac{1}{L})c_p$.
    \item By Equation \ref{eq:F_ij error}, 
    $$|\bar{F}_{ij} - F_{ij}| \leq \sqrt{Var_{\pi_i}(\psi_j^*(x))}\cdot\bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}} + \chi^2(\tilde{\pi}_i,\pi_i)^\frac{1}{2} \bigg).$$
    Then, by definition $\psi^*_j(x)\leq 1$, so we have 
    \begin{align*}
        Var_{\pi_i}(\psi_j^*(x)) &= \sqrt{\mathbb{E}_{\pi_i}\psi_j^*(x)^2 - \mathbb{E}_{\pi_i}[\psi_j^*(x)]^2}\\
&\leq \sqrt{F_{ij}(1-F_{ij})}
    \end{align*}
    Where the last line follows by the the bound on $\psi_{j}^*$ and the definition of $F_{ij} = \mathbb{E}_{\pi_i}\psi_j^*$.

Therefore, 
 $$|\bar{F}_{ij} - F_{ij}| \leq \sqrt{F_{ij}(1-F_{ij})}\cdot\bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}} + \chi^2(\tilde{\pi}_i,\pi_i)^\frac{1}{2} \bigg).$$
Since $1-F_{ij}\leq 1$
  $$|\bar{F}_{ij} - F_{ij}| \leq \sqrt{F_{ij}}\cdot\bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}} + \chi^2(\tilde{\pi}_i,\pi_i)^\frac{1}{2} \bigg).$$
  \item Combining (a) and (b) yields
  \begin{equation}
        ||\log w-\log\bar{w}||_\infty \leq \sum_{i\neq j}\frac{F_{ij}^\frac{1}{2}}{c_p^{|i-j|}}\bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}}+\chi^2(\tilde{\pi}_i,\pi_i)^\frac{1}{2}\bigg).
  \end{equation}
  To simplify, allow $\chi^2(\tilde{\pi}_i,\pi_i) \leq \epsilon_{\tilde{\pi}}$ for all $i$ then 
  \begin{equation}
      ||\log w-\log\bar{w}||_\infty \leq \bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}}+\epsilon_{\tilde{\pi}}^\frac{1}{2}\bigg)\cdot\sum_{i\neq j}\frac{F_{ij}^\frac{1}{2}}{(1-\frac{1}{L})^{|j-i|}c_p^{|i-j|}}
  \end{equation} 
  Lastly for simplification use the crude lower bound $(1-\frac{1}{L})^{|j-i|} \geq \frac{1}{4}$ for $L \geq {|j-i|}$ to get 
    \begin{equation}
      ||\log w-\log\bar{w}||_\infty \leq 4\bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}}+\epsilon_{\tilde{\pi}}^\frac{1}{2}\bigg)\cdot\sum_{i\neq j}\frac{F_{ij}^\frac{1}{2}}{c_p^{|i-j|}}
  \end{equation} 
  \note{There are two places this bound can be improved, we use $Var(X) \leq E[X^2]$ and $Q(i,j) \geq \frac{1}{2}c_p^{|j-i|}$.}
\end{enumerate}
{\bf Controlling Weight Error in the Sparse Case: } Define $F^{0}$ to be the matrix where all entries of $F$ not on the good path are zeroed out. Since $F$ is reversible $F^0$ is also reversible. Moreover, the good path assumption should guarantee that $F^{0}$ is irreducible hence the stationary distribution $w^0$ is unique, hence $w^0 = w$.

Procedurally, compute $\bar{F}$ and zero out all entries $\bar{F}_{ij}, \bar{F}_{ji}$ if both aren't greater than some $c_p$. \note{Note: the ideal criteria will be the one that gives us back only the good path.} Now the stationary distribution $\bar{w}^0$ of $\bar{F}^0$ should be a good approximate of $w^0 = w$. \note{If we can guarantee that $\bar{F}^0$ and $F^0$ have the same sparsity} then we can apply the result in the perturbation paper (equation 6) which says: 

if $F, \tilde{F}$ are irreducible stochastic matrices with $\bar{F}_{ij} = 0 \iff F_{ij} = 0$ then 

$$\max_k \max\{\frac{\tilde{\pi}_k}{\pi_k}, \frac{\pi_k}{\tilde{\pi}_k}\} \leq \bigg(\max_{i\neq j}\max\{\frac{\tilde{F}_{ij}}{F_{ij}}, \frac{F_{ij}}{\tilde{F}_{ij}}\} \bigg)^L.$$

We use previously that by choice of $N, T$ we can guarantee $|\frac{\tilde{F}_{ij}}{F_{ij}} -1| \leq \frac{1}{L}$,  here we would require a choice of $N,T$ so that $|\frac{\tilde{F}_{ij}}{F_{ij}} -1| \leq \frac{\epsilon}{L}$ this would yield a final bound on (2) of something like $\log(e^{\epsilon}) = \epsilon$.



\item {\bf Controlling sampling error  $|\log\frac{\tilde{A}_w}{\tilde{B}_w} - \log\frac{A}{B}|\leq 2 \log C_3$:}.

This reduces to $\frac{\mathbb{E}_{\tilde{\pi}_k}[f^*]}{\mathbb{E}_{\pi_k}[f^*]} \leq C_3$. Proceeding in a similar fashion to (1) yields 
$$|\log\frac{\sum_k w_k\mathbb{E}_{\tilde{\pi}_k}[f^*]}{\sum_kw_k\mathbb{E}_{\pi_k}[f^*]}|\leq \log C_3.$$

for $|\frac{w_k\mathbb{E}_{\tilde{\pi}_k}[f^*]}{w_k\mathbb{E}_{\pi_k}[f^*]}| = |\frac{\mathbb{E}_{\tilde{\pi}_k}[f^*]}{\mathbb{E}_{\pi_k}[f^*]}| \leq C_3$

Upper bound on $|\frac{\mathbb{E}_{\tilde{\pi}_k}[f^*]}{\mathbb{E}_{\pi_k}[f^*]}|$ reduces to a bound on $\chi^2(\tilde{\pi}_k, \pi_k)$ or $d_{TV}(\tilde{\pi}_k, \pi_k)$. If samples are acquired from some Markov process this will be a function of the run time. 
\item \textbf{Putting it all together:}

Using (1)-(3) yields, 

\begin{equation*}
       |\log \bar{\pi}(g) - \log \pi(g)| \leq 2\bigg( \log C_1 + C_2 + \log C_3\bigg).
\end{equation*}
With probability $1 - \delta$, Chebyshev yields, 
$$C_1 = 1+\max_i\frac{\sqrt{Var_{\tilde{\pi}_i}(f^*)}}{\mathbb{E}_{\tilde{\pi}_i}[f^*]}\cdot\sqrt{\frac{1}{N\cdot \delta}},$$
where it should be noted that this w.r.t $\tilde{\pi}_i$. 
By (2) in the to do section, with $\chi^2(\tilde{\pi}_i, \pi_i) \leq \epsilon_{\tilde{\pi}}$ for all $i$,
$$C_2 = 4\bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}}+\epsilon_{\tilde{\pi}}^\frac{1}{2}\bigg)\cdot\sum_{i\neq j}\frac{F_{ij}^\frac{1}{2}}{c_p^{|i-j|}}.$$
Lastly using Cauchy Schwarz with $\chi^2(\tilde{\pi}_i, \pi_ i) \leq \epsilon_{\tilde{\pi}}$ yields
$$C_3 = 1+\max_i\frac{\sqrt{Var_{\pi_i}(f^*)}}{\mathbb{E}_{\pi_i}f^*}\cdot\epsilon_{\tilde{\pi}}^\frac{1}{2}.$$
This should give us a rough bound of, 
\begin{equation*}
     |\log \bar{\pi}(g) - \log \pi(g)| \leq 2\bigg(\max_i\frac{\sqrt{Var_{\tilde{\pi}_i}(f^*)}}{\mathbb{E}_{\tilde{\pi}_i}[f^*]}\sqrt{\frac{1}{N\cdot \delta}}+4\bigg(\sqrt{\frac{1+\epsilon}{N\cdot\delta}}+\epsilon_{\tilde{\pi}}^\frac{1}{2}\bigg)\cdot\sum_{i\neq j}\frac{F_{ij}^\frac{1}{2}}{c_p^{|i-j|}} +\max_i\frac{\sqrt{Var_{\pi_i}(f^*)}}{\mathbb{E}_{\pi_i}f^*}\cdot\epsilon_{\tilde{\pi}}^\frac{1}{2}\bigg).
\end{equation*}

\end{enumerate}
\textbf{To Do: } Assume the following bounds exist and then show that they are satisfied for constraints on $\{\psi_i(x)\}_{i=1}^L$ and $\pi(x)$. 
\begin{enumerate}
\item With respect to the approximate measure $\tilde{\pi}_i$

$$\max_i\frac{\sqrt{Var_{\tilde{\pi}_i}(f^*)}}{\mathbb{E}_{\tilde{\pi}_i}[f^*]}\leq A_1.$$
\item With respect to the true stationary $\pi_i$ 

$$\max_i\frac{\sqrt{Var_{\pi_i}(f^*)}}{\mathbb{E}_{\pi_i}f^*} \leq A_2$$.

\item Utilizing our path assumptions 
$$\sum_{i\neq j}\frac{F_{ij}^\frac{1}{2}}{c_p^{|i-j|}}\leq A_3.$$
\end{enumerate}


==> archived.tex <==
\begin{proposition}(Relative Variance Bound) Let Assumptions \ref{a: main} and \ref{a: compact windows} hold. Let $M$ denote the maximum connectivity of the windows and let $\tilde{\pi}_i$ be an approximate to $\pi_i$ so that $\chi^2( \tilde{\pi_k} \; || \; \pi_k) \leq \tilde{\epsilon}$, as in Assumptions \ref{a: main} (2). Then 
$$ \mathcal{Q}_{\tilde{\pi}}(w,g) = \frac{\sum_jw_j\sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)} \leq \frac{M}{2c_p(1 - \frac{\sqrt{\tilde{\epsilon}}}{2})}.$$
In the case of exact sampling ($\tilde{\pi}_i = \pi_i$, we have $\epsilon = 0$, and the bound reduces to $\frac{M}{2c_p}$.
\end{proposition}
\begin{proof} Let $\mathcal{B} = \{i : 0<\pi_i(A) < 1\}$ and $\mathcal{C} = \{ i : \pi_i(A) = 1\}$ denote the set of windows on the boundary and  contained in A, respectfully. If $i \notin \mathcal{B}$ then $\pi_i(A) = 0$ or $\pi_i(A) =1$ and since $\tilde{\pi}_i$ is absolutely continuous w.r.t. $\pi_i$ this is also true of $\tilde{\pi}_i$. Therefore $\Var_{\tilde{\pi}_i}(g) = 0$ if $i \notin \mathcal{B}$. Hence
\begin{align*}
        \frac{\sum_jw_j\sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)}
        &= \sum_{j \in \mathcal{B}}\frac{w_j \sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)}
\end{align*}
Recall detailed balance of $F$ which yields $\frac{w_j}{w_i} = \frac{F_{ij}}{F_{ji}}$. By the good neighbor assumption (Assumption \ref{a: compact windows}) applied to detailed balance yields $w_j \leq \frac{w_{k(j)}}{c_p}$ for some neighbor $k(j)$ that satisfies $\mathbb{E}_{\pi_{k(j)}(g)} = 1$. Define $N(k) = \{j \in \mathcal{B} \;|\; k(j) = k\}$ to be the number of boundary windows that choose window k as their good neighbor. Then consider, 
\begin{align*}
    \sum_{j \in \mathcal{B}}\frac{w_j \sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)}\leq\frac{1}{2}\sum_{j \in \mathcal{B}}\frac{w_j}{\sum_{k \in \mathcal{C}}w_k\mathbb{E}_{\tilde{\pi}_k}(g)} \leq \frac{1}{2c_p}\sum_{k\in \mathcal{C}}\frac{ N(k)\cdot w_k}{\sum_{k \in \mathcal{C}}w_k\mathbb{E}_{\tilde{\pi}_k}(g)}. 
\end{align*}
Cauchy Schwarz yields $\lvert\mathbb{E}_{\tilde{\pi}_i}(g) - \mathbb{E}_{\pi_i}(g)\rvert \leq \sqrt{\Var_{{\pi}_i}(g)}\cdot\sqrt{\chi^2(\tilde{\pi}_i \; || \; \pi_i)}.$ Applying Assumptions \ref{a: main} (2) and recalling $\mathbb{E}_{{\pi}_k}(g) = 1$ yields $\mathbb{E}_{{\pi}_i}(g) \geq 1 - \frac{\sqrt{\tilde{\epsilon}}}{2}$.

Lastly applying the maximum connectivity of the windows for $k \in \mathcal{C}$ to the bound on the relative variance yields 
$$\frac{1}{2c_p}\sum_{k\in \mathcal{C}}\frac{ N(k)\cdot w_k }{\sum_{k \in \mathcal{C}}w_k\mathbb{E}_{\tilde{\pi}_k}(g)} \leq \frac{M}{2c_p}\frac{ \sum_{k \in\mathcal{C}} w_k }{(1 - \frac{\sqrt{\tilde{\epsilon}}}{2})\sum_{k \in \mathcal{C}}w_k} \leq \frac{M}{2c_p(1 - \frac{\sqrt{\tilde{\epsilon}}}{2})}.$$
\end{proof}

\begin{proposition}(Relative Variance Bound) Let Assumptions \ref{a: main} and \ref{a: compact windows} hold. Let $M$ denote the maximum connectivity of the windows and let $\tilde{\pi}_i$ be an approximate to $\pi_i$ so that $\chi^2( \tilde{\pi_k} \; || \; \pi_k) \leq \tilde{\epsilon}$, as in Assumptions \ref{a: main} (2). Then 
$$ \mathcal{Q}_{\tilde{\pi}}(w,g) = \frac{\sum_jw_j\sqrt{\Var_{\tilde{\pi}_j}(g^*)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g^*)} \leq \frac{M+1}{2c_p(a_p - \frac{\sqrt{\tilde{\epsilon}}}{2})}.$$
In the case of exact sampling ($\tilde{\pi}_i = \pi_i)$, we have $\epsilon = 0$, and the bound reduces to $\frac{M+1}{2c_pa_p}$.
\end{proposition}
\begin{proof} Let $\mathcal{B} = \{i : 0<\pi_i(A) < a_p\}$ and $\mathcal{C} = \{ i : \pi_i(A) > a_p\}$ denote the set of windows on the boundary and containing a significant portion of $A$, respectfully. If $i \notin \mathcal{B}\cup \mathcal{C}$ then $\pi_i(A) = 0$ and since $\tilde{\pi}_i$ is absolutely continuous w.r.t. $\pi_i$ this is also true of $\tilde{\pi}_i$. Therefore $\Var_{\tilde{\pi}_i}(g) = 0$ if $i \notin \mathcal{B}\cup\mathcal{C}$. Hence
\begin{align*}
  \frac{\sum_jw_j\sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)}
        &= \sum_{j \in \mathcal{B}}\frac{w_j \sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)} + \sum_{j \in \mathcal{C}}\frac{w_j \sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)} 
\end{align*}
We express the summation of the terms $j \in \mathcal{B}$ as a summation over the terms $j \in \mathcal{C}$. 
Recall detailed balance of $F$ which yields $\frac{w_j}{w_i} = \frac{F_{ij}}{F_{ji}}$. By the good neighbor assumption (Assumption \ref{a: compact windows}) applied to detailed balance yields $w_j \leq \frac{w_{k(j)}}{c_p}$ for some neighbor $k(j)$ that satisfies $\mathbb{E}_{\pi_{k(j)}}(g) \geq a_p$. 
Define $N(k) = \{j \in \mathcal{B} \;|\; k(j) = k \text{ and } F_{jk} \geq c_p\}$ to be the number of boundary windows that choose window k as their good neighbor. Then consider, 
\begin{align*}
    \sum_{j \in \mathcal{B}}\frac{w_j \sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)}\leq\frac{1}{2}\sum_{j \in \mathcal{B}}\frac{w_j}{\sum_{k \in \mathcal{C}}w_k\mathbb{E}_{\tilde{\pi}_k}(g)} \leq \frac{1}{2c_p}\sum_{k\in \mathcal{C}}\frac{ N(k)\cdot w_k}{\sum_{k \in \mathcal{C}}w_k\mathbb{E}_{\tilde{\pi}_k}(g)}. 
\end{align*}
Combining the two terms yields
\begin{align*}
\frac{\sum_jw_j\sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)}
        \leq \frac{1}{2c_p}\sum_{k\in \mathcal{C}}\frac{ N(k)\cdot w_k}{\sum_{k \in \mathcal{C}}w_k\mathbb{E}_{\tilde{\pi}_k}(g)} + \frac{1}{2}\sum_{j \in \mathcal{C}}\frac{w_j \sqrt{\Var_{\tilde{\pi}_j}(g)}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g)} \leq \frac{1}{2c_p}\sum_{k\in \mathcal{C}}\frac{ \left(N(k)+1\right)\cdot w_k}{\sum_{k \in \mathcal{C}}w_k\mathbb{E}_{\tilde{\pi}_k}(g)}.
\end{align*}
Cauchy Schwarz gives $\lvert\mathbb{E}_{\tilde{\pi}_i}(g) - \mathbb{E}_{\pi_i}(g)\rvert \leq \sqrt{\Var_{{\pi}_i}(g)}\cdot\sqrt{\chi^2(\tilde{\pi}_i \; || \; \pi_i)}.$ Applying Assumptions \ref{a: main} (2) and recalling for $i \in \mathcal{C}$ that $\mathbb{E}_{{\pi}_i}(g) > a_p$ yields $\mathbb{E}_{{\pi}_i}(g) > a_p - \frac{\sqrt{\tilde{\epsilon}}}{2}$.

Lastly applying the maximum connectivity of the windows for $k \in \mathcal{C}$ to the bound on the relative variance yields 

$$\frac{1}{2c_p}\sum_{k\in \mathcal{C}}\frac{ \left(N(k)+1\right)\cdot w_k }{\sum_{k \in \mathcal{C}}w_k\mathbb{E}_{\tilde{\pi}_k}(g)} \leq \frac{M+1}{2c_p}\frac{ \sum_{k \in\mathcal{C}} w_k }{(1 - \frac{\sqrt{\tilde{\epsilon}}}{2})\sum_{k \in \mathcal{C}}w_k} \leq \frac{M+1}{2c_p(1 - \frac{\sqrt{\tilde{\epsilon}}}{2})}.$$
\end{proof}

\begin{lem}\label{l: chisq subset}
  Let Assumptions \ref{a: compact windows} hold. Define $\pi_{ij} = \frac{1_{\Gamma_{ij}}}{\pi_i(\Gamma_{ij})}\pi_i$ and $\tilde{\pi}_{ij} = \frac{1_{\Gamma_{ij}}}{\tilde{\pi}_i(\Gamma_{ij})}\tilde{\pi}_i$ for windows $\psi_i(x) = 1_{W_i}(x)$. Let $\chi^2(\tilde{\pi}_i, \pi_i) \leq \tilde{\epsilon}$ and $F_{ij} = \int_\Omega \frac{\psi_j(x)}{\sum_k \psi_k(x)}\pi_i(dx)$, as in Assumptions \ref{a: main}. 
    Let $F_{ij} = \int_\Omega \frac{\psi_j(x)}{\sum_k \psi_k(x)}\pi_i(dx)$, as in Assumptions \ref{a: main}. Then 
    $$\chi^2(\tilde{\pi}_{ij}, \pi_{ij}) \leq\frac{\tilde{\epsilon}}{\left(F_{ij}^\frac{1}{2} - \tilde{\epsilon}^\frac{1}{2}\right)^2}.$$
\end{lem}
\begin{proof}
    Consider 
    \begin{align*}
\chi^2(\tilde{\pi}_{ij}, \pi_{ij}) + 1 &= \int \left( \frac{\tilde{\pi}_{ij}(x)}{\pi_{ij}(x)}\right)^2 \pi_{ij}(x) dx = \frac{\pi_i(\Gamma_{ij})}{\tilde{\pi}_{i}(\Gamma_{ij})^2}\int_{\Gamma_{ij}}\left(\frac{\tilde{\pi}_i(x)}{\pi_i(x)}\right)^2\pi_i(x)dx.
    \end{align*}
Expanding the integral term yields,
\begin{align*}
\int_{\Gamma_{ij}}\left(\frac{\tilde{\pi}_i(x)}{\pi_i(x)}\right)^2\pi_i(x)dx &= \int_{\Gamma_{ij}}\frac{\left(\tilde{\pi}_i(x)-(\pi_i(x) -\tilde{\pi}_i(x))\right)^2}{\pi_i(x)}dx\\
&= \int_{\Gamma_{ij}}\pi_i(x)dx - 2\int_{\Gamma_{ij}}\pi_i(x) - \tilde{\pi}_i(x)dx + \int_{\Gamma_{ij}}\frac{\left(\pi_i(x) -\tilde{\pi}_i(x)\right)^2}{\pi_i(x)}dx\\
&\leq 2\tilde{\pi}_i(\Gamma_{ij}) - \pi_i(\Gamma_{ij}) + \chi^2(\tilde{\pi}_i,\pi_i)
\end{align*}
Where the last inequality follows from $\int_{\Gamma_{ij}}\left(\frac{\tilde{\pi}_i(x)}{\pi_i(x)}\right)^2\pi_i(x)dx \leq \int_{W_i}\left(\frac{\tilde{\pi}_i(x)}{\pi_i(x)}\right)^2\pi_i(x)dx$. Therefore we have that 
\begin{align*}
    \chi^2(\tilde{\pi}_{ij}, \pi_{ij}) + 1 &\leq \frac{\pi_i(\Gamma_{ij})}{\tilde{\pi}_{i}(\Gamma_{ij})^2}\left(2\tilde{\pi}_i(\Gamma_{ij}) - \pi_i(\Gamma_{ij}) + \chi^2(\tilde{\pi}_i,\pi_i)\right)\\
    &= 1 - \left(1 - \frac{\pi_i(\Gamma_{ij})}{\tilde{\pi}_i(\Gamma_{ij})}\right)^2 + \frac{\pi_i(\Gamma_{ij})}{\tilde{\pi}_i(\Gamma_{ij})^2}\chi^2(\tilde{\pi}_i,\pi_i).\\
    \shortintertext{Since the squared term is always non-negative, this implies that}
        \chi^2(\tilde{\pi}_{ij}, \pi_{ij}) &\leq 1 - 1 + \frac{\pi_i(\Gamma_{ij})}{\tilde{\pi}_i(\Gamma_{ij})^2}\chi^2(\tilde{\pi}_i,\pi_i) = \frac{\pi_i(\Gamma_{ij})}{\tilde{\pi}_i(\Gamma_{ij})^2}\chi^2(\tilde{\pi}_i,\pi_i).
\end{align*}
Now we can express $\tilde{\pi}_i(\Gamma_{ij})$ as 
\begin{align*}
\tilde{\pi}_i(\Gamma_{ij})=\int_{\Gamma_{ij}}1 + \left(\frac{\tilde{\pi}_i(x)}{\pi_i(x)} -1\right)\pi_i(x)dx = \pi_i(\Gamma_{ij}) + \int_{\Gamma_{ij}}\left(\frac{\tilde{\pi}_i(x)}{\pi_i(x)} -1\right)\pi_i(x)dx \geq \pi_i(\Gamma_{ij}) - \chi^2(\tilde{\pi}_i, \pi_i)^\frac{1}{2}\pi_i(\Gamma_{ij})^\frac{1}{2}.
\end{align*}
Where the last inequality follows from $ \left|\int_{\Gamma_{ij}}\left(\frac{\tilde{\pi}_i(x)}{\pi_i(x)} -1\right)\pi_i(x)dx\right| \leq \chi^2(\tilde{\pi}_i, \pi_i)^\frac{1}{2}\pi_i(\Gamma_{ij})^\frac{1}{2}$, by Cauchy-Schwarz.
Lastly, note that 
$$F_{ij} = \int \frac{\psi_j(x)}{\sum_k \psi_k(x)}\pi_i(x) = \int 1_{W_j}\frac{1_{W_i}}{\pi(W_i)}\pi(x)=\frac{\pi(\Gamma_{ij})}{\pi(W_i)} = \pi_i(\Gamma_{ij}).$$
There using that $F_{ij} = \pi_i(\Gamma_{ij})$ and $\chi^2(\tilde{\pi}_i,\pi_i) \leq \tilde{\epsilon}$ we have
\begin{align*}
\chi^2(\tilde{\pi}_{ij}, \pi_{ij}) + 1 &\leq \frac{\pi_i(\Gamma_{ij})}{\left(\pi_i(\Gamma_{ij}) - \chi^2(\tilde{\pi}_i, \pi_i)^\frac{1}{2}\pi_i(\Gamma_{ij})^\frac{1}{2}\right)^2}\chi^2(\tilde{\pi}_i,\pi_i) \\
&\leq\frac{F_{ij}\tilde{\epsilon}}{\left(F_{ij} - \tilde{\epsilon}^\frac{1}{2}F_{ij}^\frac{1}{2}\right)^2}=\frac{\tilde{\epsilon}}{\left(F_{ij}^\frac{1}{2} - \tilde{\epsilon}^\frac{1}{2}\right)^2}.
\end{align*}
\end{proof}

\begin{lem}\label{l: Gaussian Variance Bound}(Variance Bound for Exact Sampling) Let Assumptions \ref{a: main} and \ref{a: Gaussian Windows} hold. 
Let $g: \mathbb{R}^D \rightarrow \mathbb{R}$ be an $L_g$ log-Lipschitz observable, and $\tilde{g}(z)=\mathbb{E}_\pi[g \mid \theta = z]$.
Let $L_{eff} = 2(L_g + L_S)$ so that $K \vcentcolon = C_{LS}^{(d)}L_{eff} + C_{LS}^{(\theta)} L_g^2$, if $g$ is defined only on the CV space $K = C_{LS}^{(d)}L_{eff}$, then for $K < 1$ define the variance factor 
$$\gamma \vcentcolon = \frac{K}{1-K}.$$
Then he variance under $\pi_k$ is bounded by
$$Var_{\pi_k} \left(g^*\right) \leq \gamma\mathbb{E}_{\pi_k}\left( g^*\right)^2.$$
More specifically, the weighted relative standard deviation under $\{\pi_k\}$ satisfies: 
$$\mathcal{Q}_{\{\pi\}}(w,g)\leq \gamma^\frac{1}{2}.$$
\begin{proof} Using the law of total variance, we decompose the variance as 
$$ \text{Var}_{\pi_k}(g^*) = \underbrace{\text{Var}_{\mu_k}(\mathbb{E}_{\pi_k}[g^* \mid \theta])}_{\text{Term 1: Marginal}} + \underbrace{\mathbb{E}_{\mu_k}[\text{Var}_{\pi_k}(g^* \mid \theta)]}_{\text{Term 2: Conditional}}. $$
We begin by bounding term 1. Note $\tilde{g}^*(z) = \mathbb{E}_{\pi_k}[g^* \mid \theta = z]$ since $S(x)$ is fixed for all $\theta(x) = z$, hence $\tilde{g}^*(z) = \frac{\tilde{g}(z)}{\tilde{S}(z)}$. 
\begin{align*}
   \Var_{\mu_k}(\tilde{g}^*)&\leq C_{LS}^{(d)}\mathbb{E}_{\mu_k}\left[\left\|\nabla \tilde{g}^*\right\|^2 \right] = C_{LS}^{(d)}\mathbb{E}_{\mu_k}\left[\left\|\nabla \mathbb{E}_{\pi_k}[g^* \mid \theta = z]\right\|^2 \right]\leq C_{LS}^{(d)}\mathbb{E}_{\mu_k}\left[\mathbb{E}_{\pi_k}[\|\nabla g^*\|^2 \mid \theta = z] \right].\\
   \shortintertext{Where the last inequality is given by the contracton in the Dirichlet form, see Remark \ref{r: contraction_dirichlet}. The tower property gives that this last term is exactly $C_{LS}^{(d)}\mathbb{E}_{\pi_k}[\|\nabla g^*\|^2]$. Applying Lemma \ref{l: log-Lipschitz quotient} yields}
   C_{LS}^{(d)}\mathbb{E}_{\pi_k}[\|\nabla g^*\|^2]&\leq C_{LS}^{(d)}\mathbb{E}_{\pi_k}\left[\left\|\frac{\nabla g^*}{g}\right\|^2g^*(x)^2\right]\leq C_{LS}^{(d)}(L_g + L_S)^2\mathbb{E}_{\pi_k}\left[g^*(x)^2\right] \leq C_{LS}^{(d)}L_{eff}\mathbb{E}_{\pi_k}\left[g^*(x)^2\right]. 
\end{align*}
%C_{LS}^{(d)}\mathbb{E}_{\pi_k}[\|\nabla g^*\|^2]&=C_{LS}\mathbb{E}_{\pi_k}\left[\left\|\frac{\nabla g(x)}{S(x)} - \nabla S(x)\frac{g(x)}{S(x)^2} \right\|^2\right] = C_{LS}\mathbb{E}_{\pi_k}\left[\left\|\frac{\nabla g(x)}{g(x)}\frac{g(x)}{S(x)} - \frac{\nabla S(x)}{S(x)}\frac{g(x)}{S(x)} \right\|^2\right]. 
% Cauchy-Schwarz and the Assumption that $g(x)$ and $S(x)$ are log-Lipschitz yields
% \begin{align*}
% C_{LS}^{(d)}\mathbb{E}_{\pi_k}\left[\left\|\frac{\nabla g(x)}{g(x)}\frac{g(x)}{S(x)} - \frac{\nabla S(x)}{S(x)}\frac{g(x)}{S(x)} \right\|^2\right]&\leq C_{LS}^{(d)}\mathbb{E}_{\pi_k}\left[\left\|\frac{\nabla g(x)}{g(x)} - \frac{\nabla S(x)}{S(x)} \right\|^2 g^*(x)^2\right]\\
% &\leq C_{LS}^{(d)}\mathbb{E}_{\pi_k}\left[\left(\left\|\frac{\nabla g(x)}{g(x)}\right\|^2 + \left\|\frac{\nabla S(x)}{S(x)} \right\|^2\right) g^*(x)^2\right]\\
% &\leq C_{LS}^{(d)}\left(L_g^2 + L_s^2\right)\mathbb{E}_{\pi_k}\left[ g^*(x)^2\right]\\
% &\leq  C_{LS}^{(d)}L_{eff}^2\mathbb{E}_{\pi_k}\left[ g^*(x)^2\right].
% \end{align*}
% where the last line follows from Jensen's inequality.
Term 2 is bounded by applying a Poincar\'e  inequality to

$$\Var_{\pi_k}(g^* \mid \theta = z) = \frac{1}{\tilde{S}(z)^2}\Var_{\pi_k}(g \mid \theta = z) \leq \frac{C_{LS}^{(\theta)}}{\tilde{S}(z)}\mathbb{E}_{\pi_k}\left[\|\nabla g\|^2 \mid \theta = z\right].$$
Note that if $g$ is only defined on the CV space then $\Var_{\pi_k}(g^* \mid \theta = z)  = 0$.
Then since $g$ is log-Lipschitz we have that 
$$\Var_{\pi_k}(g^* \mid \theta = z) \leq C_{LS}^{(\theta)} L_g^2\mathbb{E}_{\pi_k}\left[\frac{g^2}{\tilde{S}(z)^2} \mid \theta = z\right] = C_{LS}^{(\theta)} L_g^2 \mathbb{E}_{\pi_k}[(g^*)^2 \mid \theta = z].$$
Lastly, applying the expectation with respect to $\mu_k $ yields 
$$\mathbb{E}_{\mu_k}[\Var_{\pi_k}(g^* \mid \theta)] \leq C_{LS}^{(\theta)} L_g^2 \mathbb{E}_{\pi_k}[g^*(x)^2].$$
Combining the bounds on terms 1 and 2 gives 
$$ \text{Var}_{\pi_k}(g^*) = \text{Var}_{\mu_k}(\mathbb{E}_{\pi_k}[g^* \mid \theta]) + \mathbb{E}_{\mu_k}[\text{Var}_{\pi_k}(g^* \mid \theta)] \leq \left(C_{LS}^{(d)}L_{eff}^2 + C_{LS}^{(\theta)} L_g^2\right)\mathbb{E}_{\pi_k}[g^*(x)^2]. $$
Let $K = C_{LS}^{(d)}L_{eff}^2 + C_{LS}^{(\theta)} L_g^2$ then 
\begin{align*}
\Var_{\pi_k}(g^*) = \mathbb{E}_{\pi_k}\left[ g^*(x)^2 \right] &- \mathbb{E}_{\pi_k}\left[g^*(x) \right]^2 \leq K\mathbb{E}_{\pi_k}\left[g^*(x)^2 \right]\\
\implies \mathbb{E}_{\pi_k}\left[g^*(x)^2 \right] &\leq \frac{1}{1-K}\mathbb{E}_{\pi_k}\left[g^*(x) \right]^2.
\end{align*}
Which yields, 
\begin{equation}\label{e: var_bound}
\Var_{\pi_k}(g^*) \leq \frac{K}{1-K}\mathbb{E}_{\pi_k}\left[g^*(x)\right]^2 = \gamma \cdot \mathbb{E}_{\pi_k}\left[g^*(x)\right]^2 .
\end{equation}
Then applied to $\mathcal{Q}_{\pi}(w,g)$ we have, 
$$\mathcal{Q}_{\pi}(w,g) = \frac{\sum_k w_k\sqrt{\Var_{\pi_k}(g^*)}}{\sum_k w_k \mathbb{E}_{\pi_k}(g^*)}\leq\gamma^\frac{1}{2}\frac{\sum_k w_k \mathbb{E}_{\pi_k}(g^*)}{\sum_k w_k \mathbb{E}_{\pi_k}(g^*)} = \gamma^\frac{1}{2}.$$
\end{proof}

\begin{lem}\label{l: Gaussian Variance Bound}(Variance Bound for Exact Sampling) Let Assumptions \ref{a: main} and \ref{a: Gaussian Windows} hold. 
Let $g: \mathbb{R}^D \rightarrow \mathbb{R}$ be an $L_g$ log-Lipschitz observable, and $\tilde{g}(z)=\mathbb{E}_\pi[g \mid \theta = z]$.
Let $L_{eff}^2 = 2(L_g + L_S)^2$ so that $K \vcentcolon = \big(\Ctheta + \frac{1}{m}\Cd + \Lambda^2\Cd(\Ctheta)^2\big)L_{eff}^2$, if $g$ is defined only on the CV space $K = \frac{1}{m}C_{LS}^{(d)}L_{eff}^2$, then for $K < 1$ define the variance factor 
$$\gamma \vcentcolon = \frac{K}{1-K}.$$
Then he variance under $\pi_k$ is bounded by
$$Var_{\pi_k} \left(g^*\right) \leq \gamma\mathbb{E}_{\pi_k}\left( g^*\right)^2.$$
More specifically, the weighted relative standard deviation under $\{\pi_k\}$ satisfies: 
$$\mathcal{Q}_{\{\pi\}}(w,g)\leq \gamma^\frac{1}{2}.$$

\begin{proof} Bounding the variance we have 
\begin{align*}
   \Var_{\pi_k}({g}^*)&\leq C_{LS}^{(D)}\mathbb{E}_{\pi_k}\left[\left\|\nabla {g}^*\right\|^2 \right] = C_{LS}^{(D)}\mathbb{E}_{\pi_k}\left[\left\| \frac{\nabla{g}^*}{g^*}\right\|^2g^*(x)^2 \right]\leq C_{LS}^{(D)}L_{eff}^2\mathbb{E}_{\pi_k}\left[g^*\right].
\end{align*}
Applying the bound from Theorem 3.3, let $K = \left(\Ctheta + \frac{1}{m}\Cd + \Lambda^2\Cd(\Ctheta)^2 \right)L_{eff}^2$ then 
\begin{align*}
\Var_{\pi_k}(g^*) = \mathbb{E}_{\pi_k}\left[ g^*(x)^2 \right] &- \mathbb{E}_{\pi_k}\left[g^*(x) \right]^2 \leq K\mathbb{E}_{\pi_k}\left[g^*(x)^2 \right]\\
\implies \mathbb{E}_{\pi_k}\left[g^*(x)^2 \right] &\leq \frac{1}{1-K}\mathbb{E}_{\pi_k}\left[g^*(x) \right]^2.
\end{align*}
Which yields, 
\begin{equation}\label{e: var_bound}
\Var_{\pi_k}(g^*) \leq \frac{K}{1-K}\mathbb{E}_{\pi_k}\left[g^*(x)\right]^2 = \gamma \cdot \mathbb{E}_{\pi_k}\left[g^*(x)\right]^2 .
\end{equation}
Then applied to $\mathcal{Q}_{\pi}(w,g)$ we have, 
$$\mathcal{Q}_{\pi}(w,g) = \frac{\sum_k w_k\sqrt{\Var_{\pi_k}(g^*)}}{\sum_k w_k \mathbb{E}_{\pi_k}(g^*)}\leq\gamma^\frac{1}{2}\frac{\sum_k w_k \mathbb{E}_{\pi_k}(g^*)}{\sum_k w_k \mathbb{E}_{\pi_k}(g^*)} = \gamma^\frac{1}{2}.$$
\end{proof}

\end{lem}
\begin{lem}\label{l: Stability of Q, Gaussian}(Stability of $\mathcal{Q}$) Let the assumptions of Lemma \ref{l: Gaussian Variance Bound} hold. Let $\{\tilde{\pi}_k\}$ be the collection of biased distributions such that $\chi^2(\tilde{\pi}_k\;||\;\pi_k)< \tilde{\epsilon}$ for all k. If the sampling bias is sufficiently small such that $\tilde{\epsilon}^\frac{1}{2}\gamma^\frac{1}{2} < 1,$ then the weighted relative standard deviation under the approximate distribution satisfies: 
$$\mathcal{Q}_{\{\tilde{\pi}\}}(w,g) \leq \left[\frac{e^\frac{3C_{LS}^{(D)}\left(L_g^2+L_s^2\right)}{4}(1+\tilde{\epsilon})^\frac{1}{4}}{1-\tilde{\epsilon}^\frac{1}{2}\gamma^\frac{1}{2}} \right]\mathcal{Q}_{\{\pi\}}(w,g),$$
where $C_{LS}^{(D)} \leq \max(C_{LS}^{(d)}, C_{LS}^{(\theta)})$.
\end{lem}
\begin{proof}
    By applying Cauchy-Schwarz we can bound $\Var_{\tilde{\pi}_k}(g^*)$ in terms of $\Var_{{\pi}_i}(g^*)^2$, 
$$\Var_{\tilde{\pi}_k}(g^*) \le \E_{\tilde{\pi}_k} \left[ (g^* - \mathbb{E}_{\pi_k} g^*)^2 \right]\leq \E_{\pi_k}\left[(g^* - \mathbb{E}_{\pi_k} g^*)^4\right]^\frac{1}{2}\left(1 + \chi^2(\tilde{\pi}_k \; || \; \pi_k) \right)^\frac{1}{2}\leq\E_{\pi_k}\left[(g^* - \mathbb{E}_{\pi_k} g^*)^4\right]^\frac{1}{2}\left(1 + \tilde{\epsilon} \right)^\frac{1}{2}.$$
The biased distribution $\pi_k$ satisfies an LSI inequality with constant $C_{LS}^{(D)} \leq \max(C_{LS}^{(d)}, C_{LS}^{(\theta)})$, by Lemma \ref{l: LSI map}.
Since $g^*$ is $L_g + L_s \leq L_{eff}$ log-Lipschitz, by Lemma \ref{l: log-Lipschitz quotient}, and $\pi_k$ satisfies an LSI, Lemma \ref{l: hypercontractivity} yields 
\begin{equation}\label{e: var_ratio}
    \frac{\Var_{\tilde{\pi}_k}(g^*)}{\Var_{{\pi}_k}(g^*)}\leq \frac{\E_{\pi_k}\left[(g^* - \mathbb{E}_{\pi_k} g^*)^4\right]^\frac{1}{2}}{\mathbb{E}_{\pi_k}\left[(g^* - \mathbb{E}_{\pi_k} g^*)^2\right]}\left(1 + \tilde{\epsilon} \right)^\frac{1}{2} \leq e^{ \frac{3C_{LS}^{(D)}L_{eff}^2}{2}}\left(1 + \tilde{\epsilon} \right)^\frac{1}{2}.
\end{equation}

Similarly, we get a  lower bound on $\mathbb{E}_{\tilde{\pi}_k}(g^*)$ in terms of $\mathbb{E}_{{\pi}_k}(g^*)$ by considering, 
$$\left|\mathbb{E}_{\tilde{\pi}_k}(g^*) - \mathbb{E}_{{\pi}_k}(g^*) \right| \leq \Var_{\pi_k}(g^*)^\frac{1}{2}\cdot\chi^2(\tilde{\pi}_k \; || \; \pi_k)^\frac{1}{2} \leq \Var_{\pi_k}(g^*)^\frac{1}{2} \cdot \tilde{\epsilon}^\frac{1}{2}.$$
Using the variance bound from Lemma \ref{l: Gaussian Variance Bound},
\begin{equation}\label{e: expect}
    \mathbb{E}_{\tilde{\pi}_k}(g^*) \geq \mathbb{E}_{\pi_k}(g^*)\left(1 - \frac{\Var_\pi(g^*)^\frac{1}{2}}{\mathbb{E}_{\pi_k}(g^*)}\tilde{\epsilon}^\frac{1}{2} \right) \geq \mathbb{E}_{\pi_k}(g^*)\left(1 - \tilde{\epsilon}^\frac{1}{2}\gamma^\frac{1}{2}\right).
\end{equation}
Applying the bounds in Eq (\ref{e: var_ratio}) and Eq (\ref{e: expect}) to $\mathcal{Q}_{\{\tilde{\pi}\}}(w,g)$ yields
$$\mathcal{Q}_{\{\tilde{\pi}\}}(w,g) = \frac{\sum_kw_k\sqrt{\Var_{{\pi}_k}(g^*)\frac{\Var_{\tilde{\pi}_k}(g^*)}{\Var_{{\pi}_k}(g^*)}}}{\sum_kw_k\mathbb{E}_{\tilde{\pi}_k}(g^*)} \leq \frac{e^{ \frac{3C_{LS}^{(D)}L_{eff}^2}{4}}\left(1 + \tilde{\epsilon} \right)^\frac{1}{4}\sum_kw_k\sqrt{\Var_{{\pi}_k}(g^*)}}{\left(1 - \tilde{\epsilon}^\frac{1}{2}\gamma^\frac{1}{2}\right)\sum_kw_k\mathbb{E}_{\pi_k}(g^*)}= \frac{e^{ \frac{3C_{LS}^{(D)}(L_{eff}^2}{4}}\left(1 + \tilde{\epsilon} \right)^\frac{1}{4}}{1 - \tilde{\epsilon}^\frac{1}{2}\gamma^\frac{1}{2}}\mathcal{Q}_{\{\pi\}}(w,g).$$
\end{proof}
\begin{proof}[{Proof of Proposition \ref{p: Q bound Gaussian}}] Lemma \ref{l: Gaussian Variance Bound} and \ref{l: Stability of Q, Gaussian} split the proof of the proposition into two parts. First Lemma \ref{l: Gaussian Variance Bound} shows that $\mathcal{Q}_{\{\pi\}}(w,g)$ under the unbiased distribution can be bounded in terms of $\gamma$. Then Lemma \ref{l: Stability of Q, Gaussian} shows that $\mathcal{Q}_{\{\tilde{\pi}\}}$ can be bounded in terms of $\mathcal{Q}_{\{\pi\}}$. This provides us with a general stability result for $\mathcal{Q}$.
\begin{enumerate}
\item Lemma \ref{l: Gaussian Variance Bound} provides: 
$$\mathcal{Q}_{\{\pi\}}(w,g)\leq \gamma^\frac{1}{2}$$

\item Lemma \ref{l: Stability of Q, Gaussian} provides:
$$\mathcal{Q}_{\{\tilde{\pi}\}}(w,g) \leq \left[\frac{e^\frac{3C_{LS}^{(D)}L_{eff}^2}{4}(1+\tilde{\epsilon})^\frac{1}{4}}{1-\tilde{\epsilon}^\frac{1}{2}\gamma^\frac{1}{2}} \right]\mathcal{Q}_{\{\pi\}}(w,g).$$
\end{enumerate}
Combining these two bounds yields the result.
\end{proof}



